H.E.S.S. discovery of very high energy gamma-ray emission from PKS 0625-354

PKS 0625-354 (z=0.055) was observed with the four H.E.S.S. telescopes in 2012 during 5.5 hours. The source was detected above an energy threshold of 200 GeV at a significance level of 6.1$\sigma$. No significant variability is found in these observations. The source is well described with a power-law spectrum with photon index $\Gamma =2.84 \pm 0.50_{stat} \pm 0.10_{syst}$ and normalization (at $E_0$=1.0 TeV) $N_0(E_0)=(0.58 \pm 0.22_{stat} \pm 0.12_{syst})\times10^{-12}$ TeV$^{-1}$cm$^{-2}$s$^{-1}$. Multi-wavelength data collected with Fermi-LAT, Swift-XRT, Swift-UVOT, ATOM and WISE are also analysed. Significant variability is observed only in the Fermi-LAT $\gamma$-ray and Swift-XRT X-ray energy bands. Having a good multi-wavelength coverage from radio to very high energy, we performed a broadband modelling from two types of emission scenarios. The results from a one zone lepto-hadronic, and a multi-zone leptonic models are compared and discussed. On the grounds of energetics, our analysis favours a leptonic multi-zone model. Models associated to the X-ray variability constraint supports previous results suggesting a BL Lac nature of PKS 0625-354, with, however, a large-scale jet structure typical of a radio galaxy.

==> authors_new.tex <==

\author{H.E.S.S. Collaboration
\and H.~Abdallah \inst{1}
\and A.~Abramowski \inst{2}
\and F.~Aharonian \inst{3,4,5}
\and F.~Ait Benkhali \inst{3}
\and A.G.~Akhperjanian \inst{6,5}
\and E.O.~Ang\"uner \inst{7}
\and M.~Backes \inst{8}
\and A.~Balzer \inst{9}
\and Y.~Becherini \inst{10}
\and J.~Becker Tjus \inst{11}
\and D.~Berge \inst{12}
\and S.~Bernhard \inst{13}
\and K.~Bernl\"ohr \inst{3}
\and E.~Birsin \inst{7}
\and R.~Blackwell \inst{14}
\and M.~B\"ottcher \inst{1}
\and C.~Boisson \inst{15}
\and J.~Bolmont \inst{16}
\and P.~Bordas \inst{3}
\and J.~Bregeon \inst{17}
\and F.~Brun \inst{18}
\and P.~Brun \inst{18}
\and M.~Bryan \inst{9}
\and T.~Bulik \inst{19}
\and J.~Carr \inst{20}
\and S.~Casanova \inst{21,3}
\and N.~Chakraborty \inst{3}
\and R.~Chalme-Calvet \inst{16}
\and R.C.G.~Chaves \inst{17,22}
\and A,~Chen \inst{23}
\and J.~Chevalier \inst{24}
\and M.~Chr\'etien \inst{16}
\and S.~Colafrancesco \inst{23}
\and G.~Cologna \inst{25}
\and B.~Condon \inst{26}
\and J.~Conrad \inst{27,28}
\and C.~Couturier \inst{16}
\and Y.~Cui \inst{29}
\and I.D.~Davids \inst{1,8}
\and B.~Degrange \inst{30}
\and C.~Deil \inst{3}
\and P.~deWilt \inst{14}
\and A.~Djannati-Ata\"i \inst{31}
\and W.~Domainko \inst{3}
\and A.~Donath \inst{3}
\and L.O'C.~Drury \inst{4}
\and G.~Dubus \inst{32}
\and K.~Dutson \inst{33}
\and J.~Dyks \inst{34}
\and M.~Dyrda \inst{21}
\and T.~Edwards \inst{3}
\and K.~Egberts \inst{35}
\and P.~Eger \inst{3}
\and J.-P.~Ernenwein \inst{20}
\and P.~Espigat \inst{31}
\and C.~Farnier \inst{27}
\and S.~Fegan \inst{30}
\and F.~Feinstein \inst{17}
\and M.V.~Fernandes \inst{2}
\and D.~Fernandez \inst{17}
\and A.~Fiasson \inst{24}
\and G.~Fontaine \inst{30}
\and A.~F\"orster \inst{3}
\and S.~Funk \inst{36}
\and M.~F\"u{\ss}ling \inst{37}
\and S.~Gabici \inst{31}
\and M.~Gajdus \inst{7}
\and Y.A.~Gallant \inst{17}
\and T.~Garrigoux \inst{16}
\and G.~Giavitto \inst{37}
\and B.~Giebels \inst{30}
\and J.F.~Glicenstein \inst{18}
\and D.~Gottschall \inst{29}
\and A.~Goyal \inst{38}
\and M.-H.~Grondin \inst{26}
\and M.~Grudzi\'nska \inst{19}
\and D.~Hadasch \inst{13}
\and S.~H\"affner \inst{36}
\and J.~Hahn \inst{3}
\and J.~Hawkes \inst{14}
\and G.~Heinzelmann \inst{2}
\and G.~Henri \inst{32}
\and G.~Hermann \inst{3}
\and O.~Hervet \inst{15}
\and A.~Hillert \inst{3}
\and J.A.~Hinton \inst{3,33}
\and W.~Hofmann \inst{3}
\and P.~Hofverberg \inst{3}
\and C.~Hoischen \inst{35}
\and M.~Holler \inst{30}
\and D.~Horns \inst{2}
\and A.~Ivascenko \inst{1}
\and A.~Jacholkowska \inst{16}
\and M.~Jamrozy \inst{38}
\and M.~Janiak \inst{34}
\and F.~Jankowsky \inst{25}
\and I.~Jung-Richardt \inst{36}
\and M.A.~Kastendieck \inst{2}
\and K.~Katarzy{\'n}ski \inst{39}
\and U.~Katz \inst{36}
\and D.~Kerszberg \inst{16}
\and B.~Kh\'elifi \inst{31}
\and M.~Kieffer \inst{16}
\and J.~King \inst{3}
\and S.~Klepser \inst{37}
\and D.~Klochkov \inst{29}
\and W.~Klu\'{z}niak \inst{34}
\and D.~Kolitzus \inst{13}
\and Nu.~Komin \inst{23}
\and K.~Kosack \inst{18}
\and S.~Krakau \inst{11}
\and F.~Krayzel \inst{24}
\and P.P.~Kr\"uger \inst{1}
\and H.~Laffon \inst{26}
\and G.~Lamanna \inst{24}
\and J.~Lau \inst{14}
\and J.~Lefaucheur \inst{31}
\and V.~Lefranc \inst{18}
\and A.~Lemi\`ere \inst{31}
\and M.~Lemoine-Goumard \inst{26}
\and J.-P.~Lenain \inst{16}
\and E.~Leser \inst{35}
\and T.~Lohse \inst{7}
\and A.~Lopatin \inst{36}
\and M.~Lorentz \inst{18}
\and C.-C.~Lu \inst{3}
\and R.~Lui \inst{3}
\and V.~Marandon \inst{3}
\and A.~Marcowith \inst{17}
\and C.~Mariaud \inst{30}
\and R.~Marx \inst{3}
\and G.~Maurin \inst{24}
\and N.~Maxted \inst{17}
\and M.~Mayer \inst{7}
\and P.J.~Meintjes \inst{40}
\and U.~Menzler \inst{11}
\and M.~Meyer \inst{27}
\and A.M.W.~Mitchell \inst{3}
\and R.~Moderski \inst{34}
\and M.~Mohamed \inst{25}
\and K.~Mor{\aa} \inst{27}
\and E.~Moulin \inst{18}
\and T.~Murach \inst{7}
\and M.~de~Naurois \inst{30}
\and J.~Niemiec \inst{21}
\and L.~Oakes \inst{7}
\and H.~Odaka \inst{3}
\and S.~\"{O}ttl \inst{13}
\and S.~Ohm \inst{37}
\and B.~Opitz \inst{2}
\and M.~Ostrowski \inst{38}
\and I.~Oya \inst{37}
\and M.~Panter \inst{3}
\and R.D.~Parsons \inst{3}
\and M.~Paz~Arribas \inst{7}
\and N.W.~Pekeur \inst{1}
\and G.~Pelletier \inst{32}
\and P.-O.~Petrucci \inst{32}
\and B.~Peyaud \inst{18}
\and S.~Pita \inst{31}
\and H.~Poon \inst{3}
\and D.~Prokhorov \inst{10}
\and H.~Prokoph \inst{10}
\and G.~P\"uhlhofer \inst{29}
\and M.~Punch \inst{31,10}
\and A.~Quirrenbach \inst{25}
\and S.~Raab \inst{36}
\and I.~Reichardt \inst{31}
\and A.~Reimer \inst{13}
\and O.~Reimer \inst{13}
\and M.~Renaud \inst{17}
\and R.~de~los~Reyes \inst{3}
\and F.~Rieger \inst{3,41}
\and C.~Romoli \inst{4}
\and S.~Rosier-Lees \inst{24}
\and G.~Rowell \inst{14}
\and B.~Rudak \inst{34}
\and C.B.~Rulten \inst{15}
\and V.~Sahakian \inst{6,5}
\and D.~Salek \inst{42}
\and D.A.~Sanchez \inst{24}
\and A.~Santangelo \inst{29}
\and M.~Sasaki \inst{29}
\and R.~Schlickeiser \inst{11}
\and F.~Sch\"ussler \inst{18}
\and A.~Schulz \inst{37}
\and U.~Schwanke \inst{7}
\and S.~Schwemmer \inst{25}
\and A.S.~Seyffert \inst{1}
\and R.~Simoni \inst{9}
\and H.~Sol \inst{15}
\and F.~Spanier \inst{1}
\and G.~Spengler \inst{27}
\and F.~Spies \inst{2}
\and {\L.}~Stawarz \inst{38}
\and R.~Steenkamp \inst{8}
\and C.~Stegmann \inst{35,37}
\and F.~Stinzing \inst{36}
\and K.~Stycz \inst{37}
\and I.~Sushch \inst{1}
\and J.-P.~Tavernet \inst{16}
\and T.~Tavernier \inst{31}
\and A.M.~Taylor \inst{4}
\and R.~Terrier \inst{31}
\and M.~Tluczykont \inst{2}
\and C.~Trichard \inst{24}
\and R.~Tuffs \inst{3}
\and J.~van der Walt \inst{1}
\and C.~van~Eldik \inst{36}
\and B.~van Soelen \inst{40}
\and G.~Vasileiadis \inst{17}
\and J.~Veh \inst{36}
\and C.~Venter \inst{1}
\and A.~Viana \inst{3}
\and P.~Vincent \inst{16}
\and J.~Vink \inst{9}
\and F.~Voisin \inst{14}
\and H.J.~V\"olk \inst{3}
\and T.~Vuillaume \inst{32}
\and Z.~Wadiasingh \inst{1}
\and S.J.~Wagner \inst{25}
\and P.~Wagner \inst{7}
\and R.M.~Wagner \inst{27}
\and R.~White \inst{33,3}
\and A.~Wierzcholska \inst{25,21}
\and P.~Willmann \inst{36}
\and A.~W\"ornlein \inst{36}
\and D.~Wouters \inst{18}
\and R.~Yang \inst{3}
\and V.~Zabalza \inst{33}
\and D.~Zaborov \inst{30}
\and M.~Zacharias \inst{25}
\and A.A.~Zdziarski \inst{34}
\and A.~Zech \inst{15}
\and F.~Zefi \inst{30}
\and a.~Ziegler \inst{36}
\and N.~\.Zywucka \inst{38}
}

\institute{
Centre for Space Research, North-West University, Potchefstroom 2520, South Africa \and
Universit\"at Hamburg, Institut f\"ur Experimentalphysik, Luruper Chaussee 149, D 22761 Hamburg, Germany \and
Max-Planck-Institut f\"ur Kernphysik, P.O. Box 103980, D 69029 Heidelberg, Germany \and
Dublin Institute for Advanced Studies, 31 Fitzwilliam Place, Dublin 2, Ireland \and
National Academy of Sciences of the Republic of Armenia,  Marshall Baghramian Avenue, 24, 0019 Yerevan, Republic of Armenia  \and
Yerevan Physics Institute, 2 Alikhanian Brothers St., 375036 Yerevan, Armenia \and
Institut f\"ur Physik, Humboldt-Universit\"at zu Berlin, Newtonstr. 15, D 12489 Berlin, Germany \and
University of Namibia, Department of Physics, Private Bag 13301, Windhoek, Namibia \and
GRAPPA, Anton Pannekoek Institute for Astronomy, University of Amsterdam,  Science Park 904, 1098 XH Amsterdam, The Netherlands \and
Department of Physics and Electrical Engineering, Linnaeus University,  351 95 V\"axj\"o, Sweden \and
Institut f\"ur Theoretische Physik, Lehrstuhl IV: Weltraum und Astrophysik, Ruhr-Universit\"at Bochum, D 44780 Bochum, Germany \and
GRAPPA, Anton Pannekoek Institute for Astronomy and Institute of High-Energy Physics, University of Amsterdam,  Science Park 904, 1098 XH Amsterdam, The Netherlands \and
Institut f\"ur Astro- und Teilchenphysik, Leopold-Franzens-Universit\"at Innsbruck, A-6020 Innsbruck, Austria \and
School of Chemistry \& Physics, University of Adelaide, Adelaide 5005, Australia \and
LUTH, Observatoire de Paris, CNRS, Universit\'e Paris Diderot, 5 Place Jules Janssen, 92190 Meudon, France \and
LPNHE, Universit\'e Pierre et Marie Curie Paris 6, Universit\'e Denis Diderot Paris 7, CNRS/IN2P3, 4 Place Jussieu, F-75252, Paris Cedex 5, France \and
Laboratoire Univers et Particules de Montpellier, Universit\'e Montpellier 2, CNRS/IN2P3,  CC 72, Place Eug\`ene Bataillon, F-34095 Montpellier Cedex 5, France \and
DSM/Irfu, CEA Saclay, F-91191 Gif-Sur-Yvette Cedex, France \and
Astronomical Observatory, The University of Warsaw, Al. Ujazdowskie 4, 00-478 Warsaw, Poland \and
Aix Marseille Universi\'e, CNRS/IN2P3, CPPM UMR 7346,  13288 Marseille, France \and
Instytut Fizyki J\c{a}drowej PAN, ul. Radzikowskiego 152, 31-342 Krak{\'o}w, Poland \and
Funded by EU FP7 Marie Curie, grant agreement No. PIEF-GA-2012-332350,  \and
School of Physics, University of the Witwatersrand, 1 Jan Smuts Avenue, Braamfontein, Johannesburg, 2050 South Africa \and
Laboratoire d'Annecy-le-Vieux de Physique des Particules, Universit\'{e} Savoie Mont-Blanc, CNRS/IN2P3, F-74941 Annecy-le-Vieux, France \and
Landessternwarte, Universit\"at Heidelberg, K\"onigstuhl, D 69117 Heidelberg, Germany \and
 Universit\'e Bordeaux, CNRS/IN2P3, Centre d'\'Etudes Nucl\'eaires de Bordeaux Gradignan, 33175 Gradignan, France \and
Oskar Klein Centre, Department of Physics, Stockholm University, Albanova University Center, SE-10691 Stockholm, Sweden \and
Wallenberg Academy Fellow,  \and
Institut f\"ur Astronomie und Astrophysik, Universit\"at T\"ubingen, Sand 1, D 72076 T\"ubingen, Germany \and
Laboratoire Leprince-Ringuet, Ecole Polytechnique, CNRS/IN2P3, F-91128 Palaiseau, France \and
APC, AstroParticule et Cosmologie, Universit\'{e} Paris Diderot, CNRS/IN2P3, CEA/Irfu, Observatoire de Paris, Sorbonne Paris Cit\'{e}, 10, rue Alice Domon et L\'{e}onie Duquet, 75205 Paris Cedex 13, France \and
Univ. Grenoble Alpes, IPAG,  F-38000 Grenoble, France \\ CNRS, IPAG, F-38000 Grenoble, France \and
Department of Physics and Astronomy, The University of Leicester, University Road, Leicester, LE1 7RH, United Kingdom \and
Nicolaus Copernicus Astronomical Center, ul. Bartycka 18, 00-716 Warsaw, Poland \and
Institut f\"ur Physik und Astronomie, Universit\"at Potsdam,  Karl-Liebknecht-Strasse 24/25, D 14476 Potsdam, Germany \and
Universit\"at Erlangen-N\"urnberg, Physikalisches Institut, Erwin-Rommel-Str. 1, D 91058 Erlangen, Germany \and
DESY, D-15738 Zeuthen, Germany \and
Obserwatorium Astronomiczne, Uniwersytet Jagiello{\'n}ski, ul. Orla 171, 30-244 Krak{\'o}w, Poland \and
Centre for Astronomy, Faculty of Physics, Astronomy and Informatics, Nicolaus Copernicus University,  Grudziadzka 5, 87-100 Torun, Poland \and
Department of Physics, University of the Free State,  PO Box 339, Bloemfontein 9300, South Africa \and
Heisenberg Fellow (DFG), ITA Universität Heidelberg, Germany,  \and
GRAPPA, Institute of High-Energy Physics, University of Amsterdam,  Science Park 904, 1098 XH Amsterdam, The Netherlands}


